GastCoCo: Graph Storage and Coroutine-Based Prefetch Co-Design for Dynamic Graph Processing

An efficient data structure is fundamental to meeting the growing demands in dynamic graph processing. However, the dual requirements for graph computation efficiency (with contiguous structures) and graph update efficiency (with linked list-like structures) present a conflict in the design principles of graph structures. After experimental studies of existing state-of-the-art dynamic graph structures, we observe that the overhead of cache misses accounts for a major portion of the graph computation time. This paper presents GastCoCo, a system with graph storage and coroutine-based prefetch co-design. By employing software prefetching via stackless coroutines and introducing a prefetch-friendly data structure CBList, GastCoCo significantly alleviates the performance degradation caused by cache misses. Our results show that GastCoCo outperforms state-of-the-art graph storage systems by 1.3x - 180x in graph updates and 1.4x - 41.1x in graph computation.

==> GCbib_copy.tex <==
@inproceedings{DBLP:conf/osdi/ZhuCZM16,
  author       = {Xiaowei Zhu and
                  Wenguang Chen and
                  Weimin Zheng and
                  Xiaosong Ma},
  editor       = {Kimberly Keeton and
                  Timothy Roscoe},
  title        = {Gemini: {A} Computation-Centric Distributed Graph Processing System},
  booktitle    = {12th {USENIX} Symposium on Operating Systems Design and Implementation,
                  {OSDI} 2016, Savannah, GA, USA, November 2-4, 2016},
  pages        = {301--316},
  publisher    = {{USENIX} Association},
  year         = {2016},
  url          = {https://www.usenix.org/conference/osdi16/technical-sessions/presentation/zhu},
  timestamp    = {Tue, 02 Feb 2021 08:06:02 +0100},
  biburl       = {https://dblp.org/rec/conf/osdi/ZhuCZM16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tods/FanYXZLYLCX18,
  author       = {Wenfei Fan and
                  Wenyuan Yu and
                  Jingbo Xu and
                  Jingren Zhou and
                  Xiaojian Luo and
                  Qiang Yin and
                  Ping Lu and
                  Yang Cao and
                  Ruiqi Xu},
  title        = {Parallelizing Sequential Graph Computations},
  journal      = {{ACM} Trans. Database Syst.},
  volume       = {43},
  number       = {4},
  pages        = {18:1--18:39},
  year         = {2018},
  url          = {https://doi.org/10.1145/3282488},
  doi          = {10.1145/3282488},
  timestamp    = {Mon, 23 Jan 2023 08:15:15 +0100},
  biburl       = {https://dblp.org/rec/journals/tods/FanYXZLYLCX18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tos/KumarH20,
  author       = {Pradeep Kumar and
                  H. Howie Huang},
  title        = {GraphOne: {A} Data Store for Real-time Analytics on Evolving Graphs},
  journal      = {{ACM} Trans. Storage},
  volume       = {15},
  number       = {4},
  pages        = {29:1--29:40},
  year         = {2020},
  url          = {https://doi.org/10.1145/3364180},
  doi          = {10.1145/3364180},
  timestamp    = {Sat, 08 Jan 2022 02:22:57 +0100},
  biburl       = {https://dblp.org/rec/journals/tos/KumarH20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/GongTYYZGYYZ21,
  author       = {Shufeng Gong and
                  Chao Tian and
                  Qiang Yin and
                  Wenyuan Yu and
                  Yanfeng Zhang and
                  Liang Geng and
                  Song Yu and
                  Ge Yu and
                  Jingren Zhou},
  title        = {Automating Incremental Graph Processing with Flexible Memoization},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {14},
  number       = {9},
  pages        = {1613--1625},
  year         = {2021},
  url          = {http://www.vldb.org/pvldb/vol14/p1613-gong.pdf},
  doi          = {10.14778/3461535.3461550},
  timestamp    = {Mon, 23 Jan 2023 08:15:15 +0100},
  biburl       = {https://dblp.org/rec/journals/pvldb/GongTYYZGYYZ21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/SharmaJBLL16,
  author       = {Aneesh Sharma and
                  Jerry Jiang and
                  Praveen Bommannavar and
                  Brian Larson and
                  Jimmy Lin},
  title        = {GraphJet: Real-Time Content Recommendations at Twitter},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {9},
  number       = {13},
  pages        = {1281--1292},
  year         = {2016},
  url          = {http://www.vldb.org/pvldb/vol9/p1281-sharma.pdf},
  doi          = {10.14778/3007263.3007267},
  timestamp    = {Fri, 27 Aug 2021 11:12:55 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/SharmaJBLL16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{gupta2014real,
  author       = {Pankaj Gupta and
                  Venu Satuluri and
                  Ajeet Grewal and
                  Siva Gurumurthy and
                  Volodymyr Zhabiuk and
                  Quannan Li and
                  Jimmy Lin},
  title        = {Real-Time Twitter Recommendation: Online Motif Detection in Large
                  Dynamic Graphs},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {7},
  number       = {13},
  pages        = {1379--1380},
  year         = {2014},
  url          = {http://www.vldb.org/pvldb/vol7/p1379-lin.pdf},
  doi          = {10.14778/2733004.2733010},
  timestamp    = {Thu, 09 Mar 2023 13:29:56 +0100},
  biburl       = {https://dblp.org/rec/journals/pvldb/GuptaSGGZLL14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{zhu2019livegraph,
  author       = {Xiaowei Zhu and
                  Marco Serafini and
                  Xiaosong Ma and
                  Ashraf Aboulnaga and
                  Wenguang Chen and
                  Guanyu Feng},
  title        = {LiveGraph: {A} Transactional Graph Storage System with Purely Sequential
                  Adjacency List Scans},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {13},
  number       = {7},
  pages        = {1020--1034},
  year         = {2020},
  url          = {http://www.vldb.org/pvldb/vol13/p1020-zhu.pdf},
  doi          = {10.14778/3384345.3384351},
  timestamp    = {Tue, 23 Mar 2021 15:33:12 +0100},
  biburl       = {https://dblp.org/rec/journals/pvldb/ZhuSMACF20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{page1998winograd,
  title={Winograd., T. The pagerank citation ranking: bringing order to the web},
  author={Page, Larry and Brin, Sergey and Motwani, R},
  journal={Unpublished manuscript},
  year={1998}
}

@inproceedings{kyrola2012graphchi,
  author       = {Aapo Kyrola and
                  Guy E. Blelloch and
                  Carlos Guestrin},
  editor       = {Chandu Thekkath and
                  Amin Vahdat},
  title        = {GraphChi: Large-Scale Graph Computation on Just a {PC}},
  booktitle    = {10th {USENIX} Symposium on Operating Systems Design and Implementation,
                  {OSDI} 2012, Hollywood, CA, USA, October 8-10, 2012},
  pages        = {31--46},
  publisher    = {{USENIX} Association},
  year         = {2012},
  url          = {https://www.usenix.org/conference/osdi12/technical-sessions/presentation/kyrola},
  timestamp    = {Tue, 02 Feb 2021 08:06:00 +0100},
  biburl       = {https://dblp.org/rec/conf/osdi/KyrolaBG12.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@article{karimi2022vcsr,
  author       = {Elmira Karimi and
                  Nicolas Bohm Agostini and
                  Shi Dong and
                  David R. Kaeli},
  title        = {{VCSR:} An Efficient {GPU} Memory-Aware Sparse Format},
  journal      = {{IEEE} Trans. Parallel Distributed Syst.},
  volume       = {33},
  number       = {10},
  pages        = {3977--3989},
  year         = {2022},
  url          = {https://doi.org/10.1109/TPDS.2022.3177291},
  doi          = {10.1109/TPDS.2022.3177291},
  timestamp    = {Tue, 21 Mar 2023 21:09:51 +0100},
  biburl       = {https://dblp.org/rec/journals/tpds/KarimiADK22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{dhulipala2019low,
  author       = {Laxman Dhulipala and
                  Guy E. Blelloch and
                  Julian Shun},
  editor       = {Kathryn S. McKinley and
                  Kathleen Fisher},
  title        = {Low-latency graph streaming using compressed purely-functional trees},
  booktitle    = {Proceedings of the 40th {ACM} {SIGPLAN} Conference on Programming
                  Language Design and Implementation, {PLDI} 2019, Phoenix, AZ, USA,
                  June 22-26, 2019},
  pages        = {918--934},
  publisher    = {{ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1145/3314221.3314598},
  doi          = {10.1145/3314221.3314598},
  timestamp    = {Sun, 09 Jun 2019 19:00:05 +0200},
  biburl       = {https://dblp.org/rec/conf/pldi/DhulipalaBS19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{de2021teseo,
  author       = {Dean De Leo and
                  Peter A. Boncz},
  title        = {Teseo and the Analysis of Structural Dynamic Graphs},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {14},
  number       = {6},
  pages        = {1053--1066},
  year         = {2021},
  url          = {http://www.vldb.org/pvldb/vol14/p1053-leo.pdf},
  doi          = {10.14778/3447689.3447708},
  timestamp    = {Thu, 21 Apr 2022 17:09:21 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/LeoB21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{ediger2012stinger,
  author       = {David Ediger and
                  Robert McColl and
                  E. Jason Riedy and
                  David A. Bader},
  title        = {{STINGER:} High performance data structure for streaming graphs},
  booktitle    = {{IEEE} Conference on High Performance Extreme Computing, {HPEC} 2012,
                  Waltham, MA, USA, September 10-12, 2012},
  pages        = {1--5},
  publisher    = {{IEEE}},
  year         = {2012},
  url          = {https://doi.org/10.1109/HPEC.2012.6408680},
  doi          = {10.1109/HPEC.2012.6408680},
  timestamp    = {Sat, 19 Oct 2019 20:21:03 +0200},
  biburl       = {https://dblp.org/rec/conf/hpec/EdigerMRB12.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{fuchs2022sortledton,
  author       = {David Ediger and
                  Robert McColl and
                  E. Jason Riedy and
                  David A. Bader},
  title        = {{STINGER:} High performance data structure for streaming graphs},
  booktitle    = {{IEEE} Conference on High Performance Extreme Computing, {HPEC} 2012,
                  Waltham, MA, USA, September 10-12, 2012},
  pages        = {1--5},
  publisher    = {{IEEE}},
  year         = {2012},
  url          = {https://doi.org/10.1109/HPEC.2012.6408680},
  doi          = {10.1109/HPEC.2012.6408680},
  timestamp    = {Sat, 19 Oct 2019 20:21:03 +0200},
  biburl       = {https://dblp.org/rec/conf/hpec/EdigerMRB12.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{jaiyeoba2019graphtinker,
  author       = {Wole Jaiyeoba and
                  Kevin Skadron},
  title        = {GraphTinker: {A} High Performance Data Structure for Dynamic Graph
                  Processing},
  booktitle    = {2019 {IEEE} International Parallel and Distributed Processing Symposium,
                  {IPDPS} 2019, Rio de Janeiro, Brazil, May 20-24, 2019},
  pages        = {1030--1041},
  publisher    = {{IEEE}},
  year         = {2019},
  url          = {https://doi.org/10.1109/IPDPS.2019.00110},
  doi          = {10.1109/IPDPS.2019.00110},
  timestamp    = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl       = {https://dblp.org/rec/conf/ipps/JaiyeobaS19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{pandey2021terrace,
  author       = {Prashant Pandey and
                  Brian Wheatman and
                  Helen Xu and
                  Aydin Bulu{\c{c}}},
  editor       = {Guoliang Li and
                  Zhanhuai Li and
                  Stratos Idreos and
                  Divesh Srivastava},
  title        = {Terrace: {A} Hierarchical Graph Container for Skewed Dynamic Graphs},
  booktitle    = {{SIGMOD} '21: International Conference on Management of Data, Virtual
                  Event, China, June 20-25, 2021},
  pages        = {1372--1385},
  publisher    = {{ACM}},
  year         = {2021},
  url          = {https://doi.org/10.1145/3448016.3457313},
  doi          = {10.1145/3448016.3457313},
  timestamp    = {Thu, 09 Mar 2023 13:30:01 +0100},
  biburl       = {https://dblp.org/rec/conf/sigmod/PandeyWXB21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{jonathan2018exploiting,
  author       = {Christopher Jonathan and
                  Umar Farooq Minhas and
                  James Hunter and
                  Justin J. Levandoski and
                  Gor V. Nishanov},
  title        = {Exploiting Coroutines to Attack the "Killer Nanoseconds"},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {11},
  number       = {11},
  pages        = {1702--1714},
  year         = {2018},
  url          = {http://www.vldb.org/pvldb/vol11/p1702-jonathan.pdf},
  doi          = {10.14778/3236187.3236216},
  timestamp    = {Sat, 25 Apr 2020 13:58:50 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/JonathanMHLN18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{he2020corobase,
  author       = {Yongjun He and
                  Jiacheng Lu and
                  Tianzheng Wang},
  title        = {CoroBase: Coroutine-Oriented Main-Memory Database Engine},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {14},
  number       = {3},
  pages        = {431--444},
  year         = {2020},
  url          = {http://www.vldb.org/pvldb/vol14/p431-he.pdf},
  doi          = {10.5555/3430915.3442440},
  timestamp    = {Tue, 23 Mar 2021 16:03:22 +0100},
  biburl       = {https://dblp.org/rec/journals/pvldb/HeL020.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{chen2007improving,
  author       = {Shimin Chen and
                  Anastassia Ailamaki and
                  Phillip B. Gibbons and
                  Todd C. Mowry},
  title        = {Improving hash join performance through prefetching},
  journal      = {{ACM} Trans. Database Syst.},
  volume       = {32},
  number       = {3},
  pages        = {17},
  year         = {2007},
  url          = {https://doi.org/10.1145/1272743.1272747},
  doi          = {10.1145/1272743.1272747},
  timestamp    = {Tue, 06 Nov 2018 12:51:47 +0100},
  biburl       = {https://dblp.org/rec/journals/tods/ChenAGM07.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{kocberber2015asynchronous,
  author       = {Yusuf Onur Ko{\c{c}}berber and
                  Babak Falsafi and
                  Boris Grot},
  title        = {Asynchronous Memory Access Chaining},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {9},
  number       = {4},
  pages        = {252--263},
  year         = {2015},
  url          = {http://www.vldb.org/pvldb/vol9/p252-kocberber.pdf},
  doi          = {10.14778/2856318.2856321},
  timestamp    = {Sat, 25 Apr 2020 13:59:11 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/KocberberFG15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{conway1963design,
  author       = {Melvin E. Conway},
  title        = {Design of a separable transition-diagram compiler},
  journal      = {Commun. {ACM}},
  volume       = {6},
  number       = {7},
  pages        = {396--408},
  year         = {1963},
  url          = {https://doi.org/10.1145/366663.366704},
  doi          = {10.1145/366663.366704},
  timestamp    = {Wed, 14 Nov 2018 10:22:35 +0100},
  biburl       = {https://dblp.org/rec/journals/cacm/Conway63.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{moura2009revisiting,
  author       = {Ana L{\'{u}}cia de Moura and
                  Roberto Ierusalimschy},
  title        = {Revisiting coroutines},
  journal      = {{ACM} Trans. Program. Lang. Syst.},
  volume       = {31},
  number       = {2},
  pages        = {6:1--6:31},
  year         = {2009},
  url          = {https://doi.org/10.1145/1462166.1462167},
  doi          = {10.1145/1462166.1462167},
  timestamp    = {Wed, 14 Nov 2018 10:30:40 +0100},
  biburl       = {https://dblp.org/rec/journals/toplas/MouraI09.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@Misc{C++20,
 
howpublished = {\url{https: //www.iso.org/standard/73008.html}},
 
year = {2017},
 
title = {Technical Specification — C++ Extensions for Coroutines.},
 
author = {ISO/IEC}
 
}

@article{DBLP:journals/pvldb/GuptaSGGZLL14,
  author       = {Pankaj Gupta and
                  Venu Satuluri and
                  Ajeet Grewal and
                  Siva Gurumurthy and
                  Volodymyr Zhabiuk and
                  Quannan Li and
                  Jimmy Lin},
  title        = {Real-Time Twitter Recommendation: Online Motif Detection in Large
                  Dynamic Graphs},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {7},
  number       = {13},
  pages        = {1379--1380},
  year         = {2014},
  url          = {http://www.vldb.org/pvldb/vol7/p1379-lin.pdf},
  doi          = {10.14778/2733004.2733010},
  timestamp    = {Thu, 09 Mar 2023 13:29:56 +0100},
  biburl       = {https://dblp.org/rec/journals/pvldb/GuptaSGGZLL14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/QiuCQPZLZ18,
  author       = {Xiafei Qiu and
                  Wubin Cen and
                  Zhengping Qian and
                  You Peng and
                  Ying Zhang and
                  Xuemin Lin and
                  Jingren Zhou},
  title        = {Real-time Constrained Cycle Detection in Large Dynamic Graphs},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {11},
  number       = {12},
  pages        = {1876--1888},
  year         = {2018},
  url          = {http://www.vldb.org/pvldb/vol11/p1876-qiu.pdf},
  doi          = {10.14778/3229863.3229874},
  timestamp    = {Sat, 25 Apr 2020 13:59:16 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/QiuCQPZLZ18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/SahuMSLO17,
  author       = {Siddhartha Sahu and
                  Amine Mhedhbi and
                  Semih Salihoglu and
                  Jimmy Lin and
                  M. Tamer {\"{O}}zsu},
  title        = {The Ubiquity of Large Graphs and Surprising Challenges of Graph Processing},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {11},
  number       = {4},
  pages        = {420--431},
  year         = {2017},
  url          = {http://www.vldb.org/pvldb/vol11/p420-sahu.pdf},
  doi          = {10.1145/3186728.3164139},
  timestamp    = {Sat, 25 Apr 2020 13:58:44 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/SahuMSLO17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@conference{BolinDingKaiZengWenyuanYu,
  author = {Ding, Bolin and Zeng, Kai and Yu, Wenyuan},
  title = {Alibaba Sponsor Talk at VLDB},
  year         = {2020}
}

@inproceedings{DBLP:conf/iiswc/BeamerAP15,
  author       = {Scott Beamer and
                  Krste Asanovic and
                  David A. Patterson},
  title        = {Locality Exists in Graph Processing: Workload Characterization on
                  an Ivy Bridge Server},
  booktitle    = {2015 {IEEE} International Symposium on Workload Characterization,
                  {IISWC} 2015, Atlanta, GA, USA, October 4-6, 2015},
  pages        = {56--65},
  publisher    = {{IEEE} Computer Society},
  year         = {2015},
  url          = {https://doi.org/10.1109/IISWC.2015.12},
  doi          = {10.1109/IISWC.2015.12},
  timestamp    = {Thu, 13 Apr 2023 19:55:42 +0200},
  biburl       = {https://dblp.org/rec/conf/iiswc/BeamerAP15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/wosp/EisenmanCMCFK16,
  author       = {Assaf Eisenman and
                  Ludmila Cherkasova and
                  Guilherme Magalhaes and
                  Qiong Cai and
                  Paolo Faraboschi and
                  Sachin Katti},
  editor       = {Alberto Avritzer and
                  Alexandru Iosup and
                  Xiaoyun Zhu and
                  Steffen Becker},
  title        = {Parallel Graph Processing: Prejudice and State of the Art},
  booktitle    = {Proceedings of the 7th {ACM/SPEC} International Conference on Performance
                  Engineering, {ICPE} 2016, Delft, The Netherlands, March 12-16, 2016},
  pages        = {85--90},
  publisher    = {{ACM}},
  year         = {2016},
  url          = {https://doi.org/10.1145/2851553.2851572},
  doi          = {10.1145/2851553.2851572},
  timestamp    = {Sun, 02 Jun 2019 21:12:22 +0200},
  biburl       = {https://dblp.org/rec/conf/wosp/EisenmanCMCFK16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/asplos/CookseyJG02,
  author       = {Robert Cooksey and
                  St{\'{e}}phan Jourdan and
                  Dirk Grunwald},
  editor       = {Kourosh Gharachorloo and
                  David A. Wood},
  title        = {A stateless, content-directed data prefetching mechanism},
  booktitle    = {Proceedings of the 10th International Conference on Architectural
                  Support for Programming Languages and Operating Systems (ASPLOS-X),
                  San Jose, California, USA, October 5-9, 2002},
  pages        = {279--290},
  publisher    = {{ACM} Press},
  year         = {2002},
  url          = {https://doi.org/10.1145/605397.605427},
  doi          = {10.1145/605397.605427},
  timestamp    = {Wed, 07 Jul 2021 13:23:08 +0200},
  biburl       = {https://dblp.org/rec/conf/asplos/CookseyJG02.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/micro/CollinsSCT02,
  author       = {Jamison D. Collins and
                  Suleyman Sair and
                  Brad Calder and
                  Dean M. Tullsen},
  editor       = {Erik R. Altman and
                  Kemal Ebcioglu and
                  Scott A. Mahlke and
                  B. Ramakrishna Rau and
                  Sanjay J. Patel},
  title        = {Pointer cache assisted prefetching},
  booktitle    = {Proceedings of the 35th Annual International Symposium on Microarchitecture,
                  Istanbul, Turkey, November 18-22, 2002},
  pages        = {62--73},
  publisher    = {{ACM/IEEE} Computer Society},
  year         = {2002},
  url          = {https://doi.org/10.1109/MICRO.2002.1176239},
  doi          = {10.1109/MICRO.2002.1176239},
  timestamp    = {Sat, 30 Sep 2023 09:52:55 +0200},
  biburl       = {https://dblp.org/rec/conf/micro/CollinsSCT02.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

 @inproceedings{Roth_Moshovos_Sohi_1998,  
 title={Dependence based prefetching for linked data structures}, 
 url={http://dx.doi.org/10.1145/291069.291034}, 
 DOI={10.1145/291069.291034}, 
 booktitle={Proceedings of the eighth international conference on Architectural support for programming languages and operating systems}, 
 author={Roth, Amir and Moshovos, Andreas and Sohi, Gurindar S.}, 
 year={1998}, 
 month={Oct}, 
 language={en-US} 
 }

@inproceedings{DBLP:conf/isca/RothS99,
  author       = {Amir Roth and
                  Gurindar S. Sohi},
  editor       = {Allan Gottlieb and
                  William J. Dally},
  title        = {Effective Jump-Pointer Prefetching for Linked Data Structures},
  booktitle    = {Proceedings of the 26th Annual International Symposium on Computer
                  Architecture, {ISCA} 1999, Atlanta, Georgia, USA, May 2-4, 1999},
  pages        = {111--121},
  publisher    = {{IEEE} Computer Society},
  year         = {1999},
  url          = {https://doi.org/10.1109/ISCA.1999.765944},
  doi          = {10.1109/ISCA.1999.765944},
  timestamp    = {Fri, 24 Mar 2023 00:02:38 +0100},
  biburl       = {https://dblp.org/rec/conf/isca/RothS99.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/asplos/LukM96,
  author       = {Chi{-}Keung Luk and
                  Todd C. Mowry},
  editor       = {Bill Dally and
                  Susan J. Eggers},
  title        = {Compiler-Based Prefetching for Recursive Data Structures},
  booktitle    = {{ASPLOS-VII} Proceedings - Seventh International Conference on Architectural
                  Support for Programming Languages and Operating Systems, Cambridge,
                  Massachusetts, USA, October 1-5, 1996},
  pages        = {222--233},
  publisher    = {{ACM} Press},
  year         = {1996},
  url          = {https://doi.org/10.1145/237090.237190},
  doi          = {10.1145/237090.237190},
  timestamp    = {Mon, 28 Aug 2023 21:17:15 +0200},
  biburl       = {https://dblp.org/rec/conf/asplos/LukM96.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/hpca/EbrahimiMP09,
  author       = {Eiman Ebrahimi and
                  Onur Mutlu and
                  Yale N. Patt},
  title        = {Techniques for bandwidth-efficient prefetching of linked data structures
                  in hybrid prefetching systems},
  booktitle    = {15th International Conference on High-Performance Computer Architecture
                  {(HPCA-15} 2009), 14-18 February 2009, Raleigh, North Carolina, {USA}},
  pages        = {7--17},
  publisher    = {{IEEE} Computer Society},
  year         = {2009},
  url          = {https://doi.org/10.1109/HPCA.2009.4798232},
  doi          = {10.1109/HPCA.2009.4798232},
  timestamp    = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl       = {https://dblp.org/rec/conf/hpca/EbrahimiMP09.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@book{DBLP:series/synthesis/2014Falsafi,
  author       = {Babak Falsafi and
                  Thomas F. Wenisch},
  title        = {A Primer on Hardware Prefetching},
  series       = {Synthesis Lectures on Computer Architecture},
  publisher    = {Morgan {\&} Claypool Publishers},
  year         = {2014},
  url          = {https://doi.org/10.2200/S00581ED1V01Y201405CAC028},
  doi          = {10.2200/S00581ED1V01Y201405CAC028},
  isbn         = {978-3-031-00615-9},
  timestamp    = {Thu, 19 Oct 2023 16:45:54 +0200},
  biburl       = {https://dblp.org/rec/series/synthesis/2014Falsafi.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/PsaropoulosLMA17,
  author       = {Georgios Psaropoulos and
                  Thomas Legler and
                  Norman May and
                  Anastasia Ailamaki},
  title        = {Interleaving with Coroutines: {A} Practical Approach for Robust Index
                  Joins},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {11},
  number       = {2},
  pages        = {230--242},
  year         = {2017},
  url          = {http://www.vldb.org/pvldb/vol11/p230-psaropoulos.pdf},
  doi          = {10.14778/3149193.3149202},
  timestamp    = {Sat, 25 Apr 2020 13:58:51 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/PsaropoulosLMA17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/kdd/ZhangWLTL17,
  author       = {Chenzi Zhang and
                  Fan Wei and
                  Qin Liu and
                  Zhihao Gavin Tang and
                  Zhenguo Li},
  title        = {Graph Edge Partitioning via Neighborhood Heuristic},
  booktitle    = {Proceedings of the 23rd {ACM} {SIGKDD} International Conference on
                  Knowledge Discovery and Data Mining, Halifax, NS, Canada, August 13
                  - 17, 2017},
  pages        = {605--614},
  publisher    = {{ACM}},
  year         = {2017},
  url          = {https://doi.org/10.1145/3097983.3098033},
  doi          = {10.1145/3097983.3098033},
  timestamp    = {Fri, 25 Dec 2020 01:14:16 +0100},
  biburl       = {https://dblp.org/rec/conf/kdd/ZhangWLTL17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/hpec/WheatmanX18,
  author       = {Brian Wheatman and
                  Helen Xu},
  title        = {Packed Compressed Sparse Row: {A} Dynamic Graph Representation},
  booktitle    = {2018 {IEEE} High Performance Extreme Computing Conference, {HPEC}
                  2018, Waltham, MA, USA, September 25-27, 2018},
  pages        = {1--7},
  publisher    = {{IEEE}},
  year         = {2018},
  url          = {https://doi.org/10.1109/HPEC.2018.8547566},
  doi          = {10.1109/HPEC.2018.8547566},
  timestamp    = {Sat, 30 Sep 2023 09:42:43 +0200},
  biburl       = {https://dblp.org/rec/conf/hpec/WheatmanX18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tods/BenderH07,
  author       = {Michael A. Bender and
                  Haodong Hu},
  title        = {An adaptive packed-memory array},
  journal      = {{ACM} Trans. Database Syst.},
  volume       = {32},
  number       = {4},
  pages        = {26},
  year         = {2007},
  url          = {https://doi.org/10.1145/1292609.1292616},
  doi          = {10.1145/1292609.1292616},
  timestamp    = {Tue, 06 Nov 2018 12:51:47 +0100},
  biburl       = {https://dblp.org/rec/journals/tods/BenderH07.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/csur/Comer79,
  author       = {Douglas Comer},
  title        = {The Ubiquitous B-Tree},
  journal      = {{ACM} Comput. Surv.},
  volume       = {11},
  number       = {2},
  pages        = {121--137},
  year         = {1979},
  url          = {https://doi.org/10.1145/356770.356776},
  doi          = {10.1145/356770.356776},
  timestamp    = {Wed, 14 Nov 2018 10:31:47 +0100},
  biburl       = {https://dblp.org/rec/journals/csur/Comer79.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/kdd/StantonK12,
  author       = {Isabelle Stanton and
                  Gabriel Kliot},
  editor       = {Qiang Yang and
                  Deepak Agarwal and
                  Jian Pei},
  title        = {Streaming graph partitioning for large distributed graphs},
  booktitle    = {The 18th {ACM} {SIGKDD} International Conference on Knowledge Discovery
                  and Data Mining, {KDD} '12, Beijing, China, August 12-16, 2012},
  pages        = {1222--1230},
  publisher    = {{ACM}},
  year         = {2012},
  url          = {https://doi.org/10.1145/2339530.2339722},
  doi          = {10.1145/2339530.2339722},
  timestamp    = {Tue, 06 Nov 2018 16:59:37 +0100},
  biburl       = {https://dblp.org/rec/conf/kdd/StantonK12.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/wsdm/TsourakakisGRV14,
  author       = {Charalampos E. Tsourakakis and
                  Christos Gkantsidis and
                  Bozidar Radunovic and
                  Milan Vojnovic},
  editor       = {Ben Carterette and
                  Fernando Diaz and
                  Carlos Castillo and
                  Donald Metzler},
  title        = {{FENNEL:} streaming graph partitioning for massive scale graphs},
  booktitle    = {Seventh {ACM} International Conference on Web Search and Data Mining,
                  {WSDM} 2014, New York, NY, USA, February 24-28, 2014},
  pages        = {333--342},
  publisher    = {{ACM}},
  year         = {2014},
  url          = {https://doi.org/10.1145/2556195.2556213},
  doi          = {10.1145/2556195.2556213},
  timestamp    = {Mon, 01 May 2023 13:01:18 +0200},
  biburl       = {https://dblp.org/rec/conf/wsdm/TsourakakisGRV14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/osdi/GonzalezLGBG12,
  author       = {Joseph E. Gonzalez and
                  Yucheng Low and
                  Haijie Gu and
                  Danny Bickson and
                  Carlos Guestrin},
  editor       = {Chandu Thekkath and
                  Amin Vahdat},
  title        = {PowerGraph: Distributed Graph-Parallel Computation on Natural Graphs},
  booktitle    = {10th {USENIX} Symposium on Operating Systems Design and Implementation,
                  {OSDI} 2012, Hollywood, CA, USA, October 8-10, 2012},
  pages        = {17--30},
  publisher    = {{USENIX} Association},
  year         = {2012},
  url          = {https://www.usenix.org/conference/osdi12/technical-sessions/presentation/gonzalez},
  timestamp    = {Tue, 02 Feb 2021 08:05:56 +0100},
  biburl       = {https://dblp.org/rec/conf/osdi/GonzalezLGBG12.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/sigmod/JainLW13,
  author       = {Nilesh Jain and
                  Guangdeng Liao and
                  Theodore L. Willke},
  editor       = {Peter A. Boncz and
                  Thomas Neumann},
  title        = {GraphBuilder: scalable graph {ETL} framework},
  booktitle    = {First International Workshop on Graph Data Management Experiences
                  and Systems, {GRADES} 2013, co-located with {SIGMOD/PODS} 2013, New
                  York, NY, USA, June 24, 2013},
  pages        = {4},
  publisher    = {{CWI/ACM}},
  year         = {2013},
  url          = {http://event.cwi.nl/grades2013/04-jain.pdf},
  doi          = {10.1145/2484425.2484429},
  timestamp    = {Tue, 02 Jun 2020 13:40:26 +0200},
  biburl       = {https://dblp.org/rec/conf/sigmod/JainLW13.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nips/XieYLZ14,
  author       = {Cong Xie and
                  Ling Yan and
                  Wu{-}Jun Li and
                  Zhihua Zhang},
  editor       = {Zoubin Ghahramani and
                  Max Welling and
                  Corinna Cortes and
                  Neil D. Lawrence and
                  Kilian Q. Weinberger},
  title        = {Distributed Power-law Graph Computing: Theoretical and Empirical Analysis},
  booktitle    = {Advances in Neural Information Processing Systems 27: Annual Conference
                  on Neural Information Processing Systems 2014, December 8-13 2014,
                  Montreal, Quebec, Canada},
  pages        = {1673--1681},
  year         = {2014},
  url          = {https://proceedings.neurips.cc/paper/2014/hash/67d16d00201083a2b118dd5128dd6f59-Abstract.html},
  timestamp    = {Mon, 16 May 2022 15:41:51 +0200},
  biburl       = {https://dblp.org/rec/conf/nips/XieYLZ14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cikm/PetroniQDKI15,
  author       = {Fabio Petroni and
                  Leonardo Querzoni and
                  Khuzaima Daudjee and
                  Shahin Kamali and
                  Giorgio Iacoboni},
  editor       = {James Bailey and
                  Alistair Moffat and
                  Charu C. Aggarwal and
                  Maarten de Rijke and
                  Ravi Kumar and
                  Vanessa Murdock and
                  Timos K. Sellis and
                  Jeffrey Xu Yu},
  title        = {{HDRF:} Stream-Based Partitioning for Power-Law Graphs},
  booktitle    = {Proceedings of the 24th {ACM} International Conference on Information
                  and Knowledge Management, {CIKM} 2015, Melbourne, VIC, Australia,
                  October 19 - 23, 2015},
  pages        = {243--252},
  publisher    = {{ACM}},
  year         = {2015},
  url          = {https://doi.org/10.1145/2806416.2806424},
  doi          = {10.1145/2806416.2806424},
  timestamp    = {Mon, 26 Apr 2021 09:27:03 +0200},
  biburl       = {https://dblp.org/rec/conf/cikm/PetroniQDKI15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/AbbasKCV18,
  author       = {Zainab Abbas and
                  Vasiliki Kalavri and
                  Paris Carbone and
                  Vladimir Vlassov},
  title        = {Streaming Graph Partitioning: An Experimental Study},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {11},
  number       = {11},
  pages        = {1590--1603},
  year         = {2018},
  url          = {http://www.vldb.org/pvldb/vol11/p1590-abbas.pdf},
  doi          = {10.14778/3236187.3236208},
  timestamp    = {Sat, 25 Apr 2020 13:59:35 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/AbbasKCV18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/sigmod/PacaciO19,
  author       = {Anil Pacaci and
                  M. Tamer {\"{O}}zsu},
  editor       = {Peter A. Boncz and
                  Stefan Manegold and
                  Anastasia Ailamaki and
                  Amol Deshpande and
                  Tim Kraska},
  title        = {Experimental Analysis of Streaming Algorithms for Graph Partitioning},
  booktitle    = {Proceedings of the 2019 International Conference on Management of
                  Data, {SIGMOD} Conference 2019, Amsterdam, The Netherlands, June 30
                  - July 5, 2019},
  pages        = {1375--1392},
  publisher    = {{ACM}},
  year         = {2019},
  url          = {https://doi.org/10.1145/3299869.3300076},
  doi          = {10.1145/3299869.3300076},
  timestamp    = {Tue, 21 Mar 2023 20:57:32 +0100},
  biburl       = {https://dblp.org/rec/conf/sigmod/PacaciO19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tods/AbergerLTNOR17,
  author       = {Christopher R. Aberger and
                  Andrew Lamb and
                  Susan Tu and
                  Andres N{\"{o}}tzli and
                  Kunle Olukotun and
                  Christopher R{\'{e}}},
  title        = {EmptyHeaded: {A} Relational Engine for Graph Processing},
  journal      = {{ACM} Trans. Database Syst.},
  volume       = {42},
  number       = {4},
  pages        = {20:1--20:44},
  year         = {2017},
  url          = {https://doi.org/10.1145/3129246},
  doi          = {10.1145/3129246},
  timestamp    = {Wed, 07 Dec 2022 23:05:07 +0100},
  biburl       = {https://dblp.org/rec/journals/tods/AbergerLTNOR17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/sigmod/FuchsBG20,
  author       = {Per Fuchs and
                  Peter A. Boncz and
                  Bogdan Ghit},
  editor       = {Akhil Arora and
                  Semih Salihoglu and
                  Nikolay Yakovets},
  title        = {EdgeFrame: Worst-Case Optimal Joins for Graph-Pattern Matching in
                  Spark},
  booktitle    = {GRADES-NDA'20: Proceedings of the 3rd Joint International Workshop
                  on Graph Data Management Experiences {\&} Systems {(GRADES)} and
                  Network Data Analytics (NDA), Portland, OR, USA, June 14, 2020},
  pages        = {4:1--4:11},
  publisher    = {{ACM}},
  year         = {2020},
  url          = {https://doi.org/10.1145/3398682.3399162},
  doi          = {10.1145/3398682.3399162},
  timestamp    = {Thu, 11 Jun 2020 19:34:28 +0200},
  biburl       = {https://dblp.org/rec/conf/sigmod/FuchsBG20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/MhedhbiS19,
  author       = {Amine Mhedhbi and
                  Semih Salihoglu},
  title        = {Optimizing Subgraph Queries by Combining Binary and Worst-Case Optimal
                  Joins},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {12},
  number       = {11},
  pages        = {1692--1704},
  year         = {2019},
  url          = {http://www.vldb.org/pvldb/vol12/p1692-mhedhbi.pdf},
  doi          = {10.14778/3342263.3342643},
  timestamp    = {Sat, 25 Apr 2020 13:58:37 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/MhedhbiS19.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tpds/ChakaravarthyCM17,
  author       = {Venkatesan T. Chakaravarthy and
                  Fabio Checconi and
                  Prakash Murali and
                  Fabrizio Petrini and
                  Yogish Sabharwal},
  title        = {Scalable Single Source Shortest Path Algorithms for Massively Parallel
                  Systems},
  journal      = {{IEEE} Trans. Parallel Distributed Syst.},
  volume       = {28},
  number       = {7},
  pages        = {2031--2045},
  year         = {2017},
  url          = {https://doi.org/10.1109/TPDS.2016.2634535},
  doi          = {10.1109/TPDS.2016.2634535},
  timestamp    = {Fri, 02 Oct 2020 14:40:49 +0200},
  biburl       = {https://dblp.org/rec/journals/tpds/ChakaravarthyCM17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/dimacs/HsuRD94,
  author       = {Tsan{-}sheng Hsu and
                  Vijaya Ramachandran and
                  Nathaniel Dean},
  editor       = {Sandeep Nautam Bhatt},
  title        = {Parallel implementation of algorithms for finding connected components
                  in graphs},
  booktitle    = {Parallel Algorithms, Proceedings of a {DIMACS} Workshop, Brunswick,
                  New Jersey, USA, October 17-18, 1994},
  series       = {{DIMACS} Series in Discrete Mathematics and Theoretical Computer Science},
  volume       = {30},
  pages        = {23--41},
  publisher    = {{DIMACS/AMS}},
  year         = {1994},
  url          = {https://doi.org/10.1090/dimacs/030/02},
  doi          = {10.1090/DIMACS/030/02},
  timestamp    = {Mon, 22 May 2023 16:07:35 +0200},
  biburl       = {https://dblp.org/rec/conf/dimacs/HsuRD94.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icde/ChengYDYW08,
  author       = {Jiefeng Cheng and
                  Jeffrey Xu Yu and
                  Bolin Ding and
                  Philip S. Yu and
                  Haixun Wang},
  editor       = {Gustavo Alonso and
                  Jos{\'{e}} A. Blakeley and
                  Arbee L. P. Chen},
  title        = {Fast Graph Pattern Matching},
  booktitle    = {Proceedings of the 24th International Conference on Data Engineering,
                  {ICDE} 2008, April 7-12, 2008, Canc{\'{u}}n, Mexico},
  pages        = {913--922},
  publisher    = {{IEEE} Computer Society},
  year         = {2008},
  url          = {https://doi.org/10.1109/ICDE.2008.4497500},
  doi          = {10.1109/ICDE.2008.4497500},
  timestamp    = {Fri, 24 Mar 2023 00:00:00 +0100},
  biburl       = {https://dblp.org/rec/conf/icde/ChengYDYW08.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/FanLMTWW10,
  author       = {Wenfei Fan and
                  Jianzhong Li and
                  Shuai Ma and
                  Nan Tang and
                  Yinghui Wu and
                  Yunpeng Wu},
  title        = {Graph Pattern Matching: From Intractable to Polynomial Time},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {3},
  number       = {1},
  pages        = {264--275},
  year         = {2010},
  url          = {http://www.vldb.org/pvldb/vldb2010/pvldb\_vol3/R23.pdf},
  doi          = {10.14778/1920841.1920878},
  timestamp    = {Mon, 14 Sep 2020 15:10:40 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/FanLMTWW10.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/tods/FanWW13,
  author       = {Wenfei Fan and
                  Xin Wang and
                  Yinghui Wu},
  title        = {Incremental graph pattern matching},
  journal      = {{ACM} Trans. Database Syst.},
  volume       = {38},
  number       = {3},
  pages        = {18},
  year         = {2013},
  url          = {http://doi.acm.org/10.1145/2489791},
  doi          = {10.1145/2489791},
  timestamp    = {Fri, 10 Jun 2022 10:35:17 +0200},
  biburl       = {https://dblp.org/rec/journals/tods/FanWW13.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/aaaifs/Gallagher06,
  author       = {Brian Gallagher},
  editor       = {Ken Murray and
                  Ian Harrison},
  title        = {Matching Structure and Semantics: {A} Survey on Graph-Based Pattern
                  Matching},
  booktitle    = {Capturing and Using Patterns for Evidence Detection, Papers from the
                  2006 {AAAI} Fall Symposium, Washington, DC, USA, October 13-15, 2006},
  series       = {{AAAI} Technical Report},
  volume       = {{FS-06-02}},
  pages        = {45--53},
  publisher    = {{AAAI} Press},
  year         = {2006},
  url          = {https://www.aaai.org/Library/Symposia/Fall/2006/fs06-02-007.php},
  timestamp    = {Thu, 29 Nov 2018 17:25:49 +0100},
  biburl       = {https://dblp.org/rec/conf/aaaifs/Gallagher06.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/kdd/BecchettiBCG08,
  author       = {Luca Becchetti and
                  Paolo Boldi and
                  Carlos Castillo and
                  Aristides Gionis},
  editor       = {Ying Li and
                  Bing Liu and
                  Sunita Sarawagi},
  title        = {Efficient semi-streaming algorithms for local triangle counting in
                  massive graphs},
  booktitle    = {Proceedings of the 14th {ACM} {SIGKDD} International Conference on
                  Knowledge Discovery and Data Mining, Las Vegas, Nevada, USA, August
                  24-27, 2008},
  pages        = {16--24},
  publisher    = {{ACM}},
  year         = {2008},
  url          = {https://doi.org/10.1145/1401890.1401898},
  doi          = {10.1145/1401890.1401898},
  timestamp    = {Fri, 09 Apr 2021 18:36:42 +0200},
  biburl       = {https://dblp.org/rec/conf/kdd/BecchettiBCG08.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/Fan22,
  author       = {Wenfei Fan},
  title        = {Big Graphs: Challenges and Opportunities},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {15},
  number       = {12},
  pages        = {3782--3797},
  year         = {2022},
  url          = {https://www.vldb.org/pvldb/vol15/p3782-fan.pdf},
  doi          = {10.14778/3554821.3554899},
  timestamp    = {Mon, 23 Oct 2023 15:31:38 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/Fan22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1912-12740,
  author       = {Maciej Besta and
                  Marc Fischer and
                  Vasiliki Kalavri and
                  Michael Kapralov and
                  Torsten Hoefler},
  title        = {Practice of Streaming and Dynamic Graphs: Concepts, Models, Systems,
                  and Parallelism},
  journal      = {CoRR},
  volume       = {abs/1912.12740},
  year         = {2019},
  url          = {http://arxiv.org/abs/1912.12740},
  eprinttype    = {arXiv},
  eprint       = {1912.12740},
  timestamp    = {Sat, 04 Jan 2020 19:40:16 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1912-12740.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/sigmod/WeiYLL16,
  author       = {Hao Wei and
                  Jeffrey Xu Yu and
                  Can Lu and
                  Xuemin Lin},
  editor       = {Fatma {\"{O}}zcan and
                  Georgia Koutrika and
                  Sam Madden},
  title        = {Speedup Graph Processing by Graph Ordering},
  booktitle    = {Proceedings of the 2016 International Conference on Management of
                  Data, {SIGMOD} Conference 2016, San Francisco, CA, USA, June 26 -
                  July 01, 2016},
  pages        = {1813--1828},
  publisher    = {{ACM}},
  year         = {2016},
  url          = {https://doi.org/10.1145/2882903.2915220},
  doi          = {10.1145/2882903.2915220},
  timestamp    = {Thu, 20 Apr 2023 20:53:53 +0200},
  biburl       = {https://dblp.org/rec/conf/sigmod/WeiYLL16.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/vldb/AilamakiDHW99,
  author       = {Anastassia Ailamaki and
                  David J. DeWitt and
                  Mark D. Hill and
                  David A. Wood},
  editor       = {Malcolm P. Atkinson and
                  Maria E. Orlowska and
                  Patrick Valduriez and
                  Stanley B. Zdonik and
                  Michael L. Brodie},
  title        = {DBMSs on a Modern Processor: Where Does Time Go?},
  booktitle    = {VLDB'99, Proceedings of 25th International Conference on Very Large
                  Data Bases, September 7-10, 1999, Edinburgh, Scotland, {UK}},
  pages        = {266--277},
  publisher    = {Morgan Kaufmann},
  year         = {1999},
  url          = {http://www.vldb.org/conf/1999/P28.pdf},
  timestamp    = {Wed, 11 May 2022 08:53:25 +0200},
  biburl       = {https://dblp.org/rec/conf/vldb/AilamakiDHW99.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{he2023graphscope,
  title={GraphScope Flex: LEGO-like Graph Computing Stack},
  author={He, Tao and Hu, Shuxian and Lai, Longbin and Li, Dongze and Li, Neng and Li, Xue and Liu, Lexiao and Luo, Xiaojian and Lyu, Binqing and Meng, Ke and others},
  journal={arXiv preprint arXiv:2312.12107},
  year={2023}
}

@inproceedings{DBLP:conf/icde/MackoMMS15,
  author       = {Peter Macko and
                  Virendra J. Marathe and
                  Daniel W. Margo and
                  Margo I. Seltzer},
  editor       = {Johannes Gehrke and
                  Wolfgang Lehner and
                  Kyuseok Shim and
                  Sang Kyun Cha and
                  Guy M. Lohman},
  title        = {{LLAMA:} Efficient graph analytics using Large Multiversioned Arrays},
  booktitle    = {31st {IEEE} International Conference on Data Engineering, {ICDE} 2015,
                  Seoul, South Korea, April 13-17, 2015},
  pages        = {363--374},
  publisher    = {{IEEE} Computer Society},
  year         = {2015},
  url          = {https://doi.org/10.1109/ICDE.2015.7113298},
  doi          = {10.1109/ICDE.2015.7113298},
  timestamp    = {Thu, 23 Mar 2023 23:59:58 +0100},
  biburl       = {https://dblp.org/rec/conf/icde/MackoMMS15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2004-00803,
  author       = {Guanyu Feng and
                  Zixuan Ma and
                  Daixuan Li and
                  Xiaowei Zhu and
                  Yanzheng Cai and
                  Wentao Han and
                  Wenguang Chen},
  title        = {RisGraph: {A} Real-Time Streaming System for Evolving Graphs},
  journal      = {CoRR},
  volume       = {abs/2004.00803},
  year         = {2020},
  url          = {https://arxiv.org/abs/2004.00803},
  eprinttype    = {arXiv},
  eprint       = {2004.00803},
  timestamp    = {Wed, 08 Apr 2020 17:08:25 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2004-00803.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/pvldb/LeoB21,
  author       = {Dean De Leo and
                  Peter A. Boncz},
  title        = {Teseo and the Analysis of Structural Dynamic Graphs},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {14},
  number       = {6},
  pages        = {1053--1066},
  year         = {2021},
  url          = {http://www.vldb.org/pvldb/vol14/p1053-leo.pdf},
  doi          = {10.14778/3447689.3447708},
  timestamp    = {Thu, 21 Apr 2022 17:09:21 +0200},
  biburl       = {https://dblp.org/rec/journals/pvldb/LeoB21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@book{DBLP:books/daglib/0009092,
  author       = {Yousef Saad},
  title        = {Iterative methods for sparse linear systems},
  publisher    = {{SIAM}},
  year         = {2003},
  url          = {https://doi.org/10.1137/1.9780898718003},
  doi          = {10.1137/1.9780898718003},
  isbn         = {978-0-89871-534-7},
  timestamp    = {Tue, 16 May 2017 14:01:41 +0200},
  biburl       = {https://dblp.org/rec/books/daglib/0009092.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/nsdi/FanAK13,
  author       = {Bin Fan and
                  David G. Andersen and
                  Michael Kaminsky},
  editor       = {Nick Feamster and
                  Jeffrey C. Mogul},
  title        = {MemC3: Compact and Concurrent MemCache with Dumber Caching and Smarter
                  Hashing},
  booktitle    = {Proceedings of the 10th {USENIX} Symposium on Networked Systems Design
                  and Implementation, {NSDI} 2013, Lombard, IL, USA, April 2-5, 2013},
  pages        = {371--384},
  publisher    = {{USENIX} Association},
  year         = {2013},
  url          = {https://www.usenix.org/conference/nsdi13/technical-sessions/presentation/fan},
  timestamp    = {Tue, 02 Feb 2021 08:05:05 +0100},
  biburl       = {https://dblp.org/rec/conf/nsdi/FanAK13.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/cbm/AzadifarRBMO22,
  author       = {Saeid Azadifar and
                  Mehrdad Rostami and
                  Kamal Berahmand and
                  Parham Moradi and
                  Mourad Oussalah},
  title        = {Graph-based relevancy-redundancy gene selection method for cancer
                  diagnosis},
  journal      = {Comput. Biol. Medicine},
  volume       = {147},
  pages        = {105766},
  year         = {2022},
  url          = {https://doi.org/10.1016/j.compbiomed.2022.105766},
  doi          = {10.1016/J.COMPBIOMED.2022.105766},
  timestamp    = {Mon, 24 Oct 2022 20:51:24 +0200},
  biburl       = {https://dblp.org/rec/journals/cbm/AzadifarRBMO22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cikm/TuQWZLZWZZ23,
  author       = {Ke Tu and
                  Wei Qu and
                  Zhengwei Wu and
                  Zhiqiang Zhang and
                  Zhongyi Liu and
                  Yiming Zhao and
                  Le Wu and
                  Jun Zhou and
                  Guannan Zhang},
  editor       = {Ingo Frommholz and
                  Frank Hopfgartner and
                  Mark Lee and
                  Michael Oakes and
                  Mounia Lalmas and
                  Min Zhang and
                  Rodrygo L. T. Santos},
  title        = {Disentangled Interest importance aware Knowledge Graph Neural Network
                  for Fund Recommendation},
  booktitle    = {Proceedings of the 32nd {ACM} International Conference on Information
                  and Knowledge Management, {CIKM} 2023, Birmingham, United Kingdom,
                  October 21-25, 2023},
  pages        = {2482--2491},
  publisher    = {{ACM}},
  year         = {2023},
  url          = {https://doi.org/10.1145/3583780.3614846},
  doi          = {10.1145/3583780.3614846},
  timestamp    = {Wed, 13 Dec 2023 14:06:02 +0100},
  biburl       = {https://dblp.org/rec/conf/cikm/TuQWZLZWZZ23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/information/ZaminiRR22,
  author       = {Mohamad Zamini and
                  Hassan Reza and
                  Minou Rabiei},
  title        = {A Review of Knowledge Graph Completion},
  journal      = {Inf.},
  volume       = {13},
  number       = {8},
  pages        = {396},
  year         = {2022},
  url          = {https://doi.org/10.3390/info13080396},
  doi          = {10.3390/INFO13080396},
  timestamp    = {Tue, 18 Oct 2022 22:18:09 +0200},
  biburl       = {https://dblp.org/rec/journals/information/ZaminiRR22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Livejournal_dataset,
  title={Group formation in large social networks: membership, growth, and evolution},
  author={Backstrom, Lars and Huttenlocher, Dan and Kleinberg, Jon and Lan, Xiangyang},
  booktitle={Proceedings of the 12th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={44--54},
  year={2006}
}

@inproceedings{Hollywood_dataset,
  author = "Paolo Boldi and Sebastiano Vigna",
  title = "The {W}eb{G}raph Framework {I}: {C}ompression Techniques",
  year = 2004,
  booktitle = "Proc. of the Thirteenth International World Wide Web Conference (WWW 2004)",
  address = "Manhattan, USA",
  pages = "595--601",
  publisher = "ACM Press"
}

@article{DBLP:journals/computer/Smith78,
  author       = {Alan Jay Smith},
  title        = {Sequential Program Prefetching in Memory Hierarchies},
  journal      = {Computer},
  volume       = {11},
  number       = {12},
  pages        = {7--21},
  year         = {1978},
  url          = {https://doi.org/10.1109/C-M.1978.218016},
  doi          = {10.1109/C-M.1978.218016},
  timestamp    = {Wed, 12 Aug 2020 10:29:41 +0200},
  biburl       = {https://dblp.org/rec/journals/computer/Smith78.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/sc/BaerC91,
  author       = {Jean{-}Loup Baer and
                  Tien{-}Fu Chen},
  editor       = {Joanne L. Martin},
  title        = {An effective on-chip preloading scheme to reduce data access penalty},
  booktitle    = {Proceedings Supercomputing '91, Albuquerque, NM, USA, November 18-22,
                  1991},
  pages        = {176--186},
  publisher    = {{ACM}},
  year         = {1991},
  url          = {https://doi.org/10.1145/125826.125932},
  doi          = {10.1145/125826.125932},
  timestamp    = {Wed, 16 Oct 2019 14:14:57 +0200},
  biburl       = {https://dblp.org/rec/conf/sc/BaerC91.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@manual{Intel2016,
  title        = {Intel 64 and IA-32 Architectures Software Developer Manuals},
  author       = {{Intel Corporation}},
  year         = 2016,
  month        = Oct,
  note         = {(Oct. 2016)},
}

@article{nips19joint,
  title={Joint optimization of tree-based index and deep model for recommender systems},
  author={Zhu, Han and Chang, Daqing and Xu, Ziru and Zhang, Pengye and Li, Xiang and He, Jie and Li, Han and Xu, Jian and Gai, Kun},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  year={2019}
}

@article{callahan1991software,
  title={Software prefetching},
  author={Callahan, David and Kennedy, Ken and Porterfield, Allan},
  journal={ACM SIGARCH Computer Architecture News},
  volume={19},
  number={2},
  pages={40--52},
  year={1991},
  publisher={ACM New York, NY, USA}
}

@article{corograph,
  author       = {Zhi, Xiangyu and Yan, Xiao and Tang, Bo and Yin, Ziyao and Zhu, Yanchao and Zhou, Minqi},
  title        = {CoroGraph: Bridging Cache Efficiency and Work Efficiency for Graph Algorithm Execution},
  journal      = {Proc. {VLDB} Endow.},
  volume       = {17},
  number       = {4},
  pages        = {891--903},
  year         = {2024}
}


==> secx-adapt-abort.tex <==
\section{Hybrid Prefetching}
\label{sec:adapt-layer}

% \subsection{Coroutine Number}


% \begin{algorithm}
% \DontPrintSemicolon
% \caption{Prefetch Strategies}
% \label{alg:pre_strategy}

% \SetKwFunction{Fallhard}{GetNeighbors\_AllHard}
% \SetKwFunction{Fallsoft}{GetNeighbors\_AllSoft}
% \SetKwFunction{FHN}{GetNeighbors\_HybridByN}
% \SetKwFunction{FHV}{GetNeighbors\_HybridByV}
% \SetKwFunction{Fprefetch}{prefetch}
% \SetKwFunction{Fcompute}{compute}
% \SetKwProg{Fn}{Function}{:}{}
% \SetKwFor{For}{for}{do}{endfor}
% \SetKw{KwTo}{to}

% \Fn{\Fallhard{$vertex$}}{
%     $n \gets vertex.chunk\_num$\;
%     $ptr \gets vertex.Traversal$\;
%     \For{\( i \gets 1 \) \KwTo \( n \)}{
%         \Fcompute{$ptr$}\;
%         $ptr \gets ptr.next$\;
%     }
% }
% \;
% \Fn{\Fallsoft{$vertex$}}{
%     $n \gets vertex.chunk\_num$\;
%     $ptr \gets vertex.Traversal$\;
%     \For{\( i \gets 1 \) \KwTo \( n \)}{
%         \Fprefetch{$ptr$}\;
%         co\_await \textbf{suspend\_always}\;
%         \Fcompute{$ptr$}\;
%         $ptr \gets ptr.next$\;
%     }
% }
% \;
% \Fn{\FHN{$vertex, loop\_N$}}{
%     $n \gets vertex.chunk\_num$\;
%     $ptr \gets vertex.Traversal$\;
%     \For{\( i \gets 1 \) \KwTo \( n \)}{
%         \If{$i < loop\_N$}{
%             \Fprefetch{$ptr$}\;
%             co\_await \textbf{suspend\_always}\;
%         }
%         \Fcompute{$ptr$}\;
%         $ptr \gets ptr.next$\;
%     }
% }
% \;
% \Fn{\FHV{$vertex, threshold\_level$}}{
%     $n \gets vertex.chunk\_num$\;
%     $ptr \gets vertex.Traversal$\;
%     \If{$vertex.level < threshold\_level$}{
%         \For{\( i \gets 1 \) \KwTo \( n \)}{
%             \Fcompute{$ptr$}\;
%             $ptr \gets ptr.next$\;
%         }
%     }
%     \Else{
%         \For{\( i \gets 1 \) \KwTo \( n \)}{
%             \Fprefetch{$ptr$}\;
%             co\_await \textbf{suspend\_always}\;
%             \Fcompute{$ptr$}\;
%             $ptr \gets ptr.next$\;
%         }
%     }
% }

% \end{algorithm}

\begin{figure}[t]
  \centering
  \includegraphics[width=2.5in]{fig-sec6/hybrid_strategy.pdf}
  \caption{Hybrid strategy. (In this example, we assume that blocks C and F will be successfully prefetched by hardware prefetchers.)}
  \label{fig:hybrid_strategy}
\end{figure}

Hardware prefetching fetches data that is silent to users.
However, if hardware prefetching succeeds, repeatedly operating software prefetching would lead to an additional overhead.
Accordingly, different strategies may influence the efficiency of different patterns of accessing vertices and edges.

We consider the phenomenon caused by the skewed graph structures from three perspectives:
\ding{172} Array-like structures certainly offer good performance for computation, but frequent update requirements can limit their use. 
\ding{173} Hardware prefetching can also be effective on linked list-like structures, but fetching the front blocks of a linked list will cause cache misses.
When it comes to the graphs where most vertices are low-degree (linked lists storing neighborhood are very short), the jump-pointer mechanism cannot take effect in time on most linked lists \zyf{don't get it. rewrite}, thus dramatically increasing the time cost.
\ding{174} Maintaining ordered data is also necessary for graph queries and GPM, so tree-like structures are needed. 
However, hardware prefetching does not work effectively on them.

% \todo{lhf:see comments.}
%lhf:预取同一棵树的时候，何时需要放弃软件预取？（实现思路：通过时间戳？LRU？可能只为度数Top的Hub Vertex设计？）

An ideal collaborative state is to use software prefetching when the hardware prefetching fails to fetch data and to avoid using software prefetching when hardware prefetching is effective.
Thus, we choose to design different and hybrid strategies for specific patterns to perform better, as shown in \autoref{fig:hybrid_strategy}. 

Firstly, we propose two basic strategies, namely \emph{All Hard} and \emph{All Soft}, according to whether to use the soft prefetching or not.
The strategy \emph{All Hard} uses hardware prefetching exclusively. 
In real-world graph data, most vertices in \ourstorage exhibit only a single or very few adjacent edge blocks (due to the skewness of the graphs).
This makes it difficult to distinguish the preparation time of hardware prefetching during \PrAllNeis on one vertex.
In the case of \PrAllVs, we utilize the GTChain to combine multiple low-degree vertices into longer chains, thus providing more preparation time for hardware prefetching. 

\emph{All Soft} employs software prefetching exclusively.
Although may conflict with hardware prefetching across various tasks, it was proven to be an effective strategy, as proposed in the experiments.
% However, in \PrAllVsCond or \PrOneV, the prefetching strategy sometimes results in poor performance.


As for the edge access patterns, we can discern the effectiveness of hardware prefetching and design a suitable hybrid strategy for prefetching. 

\textbf{Strategy for \PrOneNei.}
For the pattern \PrOneNei, since each interval tree node usually contains more than one child node, it is difficult to predict and perform prefetching operations for hardware prefetching.
Therefore, we consider using the software prefetching strategy \emph{All Soft} exclusively.
% Our experimental results also validate the inefficiency of hardware prefetching. 

\textbf{Strategies for \PrAllNeis.}
For the pattern \PrAllNeis, it needs to traverse GTChain (or part) containing several chunks or leaf nodes. 
From \autoref{subsec:cache_miss_and_hard_pre}, the jump-pointer mechanism requires the preparation time at the beginning blocks of the linked list which is not inefficient.
%in this type of linked-list traversal, i.e., hardware prefetching is not effective in the first few blocks of the list. 
The preparation time is highly related to the capability of data fetching across different CPUs.
% The specific amount of 'Preparation Time' required varies across different CPUs and relates to their prefetching capabilities. 
To this end, we propose two hybrid strategies, \emph{Hybrid I} and \emph{Hybrid II}, the pseudocodes of which are shown in \autoref{alg:pre_strategy}.
In practice, there may be situations where multiple strategies are employed concurrently.

\emph{Hybrid I strategy with hardware failure time.}
The strategy uses software prefetching for the first $N$ blocks when traversing the chain, and switches to hardware prefetching from the $N+1$th block onwards. 
The selection of $N$ can be based on the block number where hardware prefetching starts to show convergence in performance. 
This strategy, although it seems cumbersome to implement compared with the basic strategies (as it requires measuring $N$), is regarded as an efficient and flexible solution in consideration of both software and hardware prefetching.

\emph{Hybrid II strategy with the content to be prefetched.}
This strategy chooses the prefetching method based on the volume of the content to be prefetched. 
If the volume of content is relatively small, the cost of using software prefetching will exceed its benefit. 
Therefore, we choose to use hardware prefetching for small-volume content and switch to software prefetching for large-volume content. 
More specifically, in \ourstorage, the size of any block is fixed as the multiple of the Cache line size.
We can easily determine the upper bound of the prefetch content volume based on the size (or level) of the block to be accessed.
We tend to use hardware prefetching for small chunk blocks and use software prefetching for B+ tree nodes.
